Discrete intrinsic volumes

For a convex lattice polytope $P\subset \mathbb R^d$ of dimension $d$ with vertices in $\mathbb Z^d$, denote by $L(P)$ its discrete volume which is defined as the number of integer points inside $P$. The classical result due to Ehrhart says that for a positive integer $n$, the function $L(nP)$ is a polynomial in $n$ of degree $d$ whose leading coefficient is the volume of $P$. In particular, $L(nP)$ approximates the volume of $nP$ for large $n$. In convex geometry, one of the central notion which generalizes the volume is the intrinsic volumes. The main goal of this paper is to introduce their discrete counterparts. In particular, we show that for them the analogue of the Ehrhart result holds, where the volume is replaced by the intrinsic volume. We also introduce and study a notion of Grassmann valuation which generalizes both the discrete volume and the solid-angle valuation introduced by Reeve and Macdonald.

==> abstract.tex <==
В данной работе рассмотрены различные свойства выпуклых многогранников с вершинами в целочисленной решетке. А именно, представлен дискретный аналог k-ого внутреннего объема такого многогранника P (который мы назвали k-ым дискретным внутренним объемом), являющийся аддитивной функцией на множестве всех выпуклых решетчатых многогранников, и изучены его свойства. В частности, доказано предельное равенство при n стремящемся к бесконечности k-ого внутреннего объема многогранника nP (n - натуральное число) и  дискретного k-ого внутреннего объема nP. Как следствие аддитивности, дискретный k-ый внутренний объем многогранника nP для фиксированного P является многочленом от n. Этот результат является своего рода обобщением дискретного объема выпуклого решетчатого многогранника, впервые рассмотренного Эрхартом.

Другим результатом данной работы является еще одно обобщение, позволяющее связать сразу два ранее известных способа определения дискретных объемов: как количество точек решетки в многограннике и как сумму по точкам решетки телесных углов касательных конусов к многограннику в этих точках. Таким обобщением служит решетчатая сумма введенных нами модифицированных грассмановых углов многогранника в целочисленных точках. Изучены свойства этой обобщающей функции и доказано, что модифицированное определение грассмановых углов связано с исходным, причем именно новое определение, в отличие от исходного, влечет аддитивность обобщающей функции на множестве выпуклых решетчатых многогранников. Более того, новое определение само по себе удобнее во многих случаях, что также отражено в работе.

In the thesis, we consider different properties of convex polytopes with vertices in an integer lattice. Namely, we present a discrete analogue of the k-th intrinsic volume of such a polytope P (we called it the k-th discrete intrinsic volume), which is an additive function on the set of all convex lattice polytopes, and study its properties. In particular, we showed an asymptotic equality as n tends to infinity of the k-th intrinsic volume of the polytope nP (n is a natural number) and the k-th discrete intrinsic volume of nP. As a consequence of the additivity, the k-th discrete intrinsic volume of the polytope nP for a fixed P is a polynomial in n. This result is a kind of generalization of the discrete volume of the convex lattice polytope first considered by Ehrhart.

Another result of this thesis is one more generalization that allows one to connect two previously known methods for determining discrete volumes at once: as the number of lattice points in a polytope and as the sum over the lattice points of the solid angles of tangent cones to the polytope at these points. Such a generalization is the lattice sum of the introduced by us modified Grassmann angles of the polytope at the integer points. The properties of this generalizing function are studied and it is proved that the modified definition of Grassmann angles is related to the original one, and it is the new definition, in contrast to the original one, that implies the additivity of the generalizing function on the set of convex lattice polytopes. Moreover, the new definition itself is more convenient in many cases, which is also considered in the paper.

Key words: lattice polytope, discrete volume, intrinsic volume, discrete intrinsic volume, conic intrinsic volume, Grassmann angle, Ehrhart polynomial, solid-angle polynomial, solid angle, valuation.

==> def.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{amsmath}% amstex ?
\usepackage{amsthm}
\usepackage{amssymb,bbm}%
\usepackage[numbers, square]{natbib}



%Theorems***************************************
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{observation}[thm]{Observation}
\newtheorem{problem}[thm]{Problem}
\newtheorem{question}[thm]{Question}

\theoremstyle{definition}
\newtheorem{definition}[thm]{Definition}
\newtheorem{notation}[thm]{Notation}
\newtheorem{example}{Example}

\theoremstyle{remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{convention}[thm]{Convention}
\newtheorem{claim}[thm]{Claim}
\makeindex
\makeglossary

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\Sd}{\mathbb{S}^{d-1}}
\newcommand{\bV}{\mathbb{\hspace{-.07mm}V\hspace{-.2mm}}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}

\newcommand{\E}{\mathbb E\,}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\s}{\mathbb{S}}
\newcommand{\B}{\mathbb{B}}
\renewcommand{\P}{\mathbb{P}}
%\mathrm commands
\newcommand{\Var}{\mathop{\mathrm{Var}}\nolimits}
\newcommand{\Int}{\mathop{\mathrm{int}}\nolimits}
\newcommand{\cl}{\mathop{\mathrm{cl}}\nolimits}
\newcommand{\bd}{\mathop{\mathrm{bd}}\nolimits}
\newcommand{\relint}{\mathop{\mathrm{relint}}\nolimits}
\newcommand{\relcl}{\mathop{\mathrm{relcl}}\nolimits}
\newcommand{\relbd}{\mathop{\mathrm{relbd}}\nolimits}
\newcommand{\Vol}{\mathop{\mathrm{Vol}}\nolimits}
\newcommand{\supp}{\mathop{\mathrm{supp}}\nolimits}
\newcommand{\Cov}{\mathop{\mathrm{Cov}}\nolimits}
\newcommand{\conv}{{\mathrm{conv}}}
\newcommand{\cone}{\mathop{\mathrm{cone}}\nolimits}
\newcommand{\spec}{\mathop{\mathrm{spec}}\nolimits}
\newcommand{\pos}{\mathop{\mathrm{pos}}\nolimits}
\newcommand{\lin}{\mathop{\mathrm{lin}}\nolimits}
\newcommand{\aff}{\mathop{\mathrm{aff}}\nolimits}
\newcommand{\dist}{\mathop{\mathrm{dist}}\nolimits}
\newcommand{\diam}{\mathop{\mathrm{diam}}\nolimits}
\newcommand{\Span}{\mathop{\mathrm{span}}\nolimits}
\newcommand{\rank}{\mathop{\mathrm{rank}}\nolimits}
\newcommand{\codim}{\mathop{\mathrm{codim}}\nolimits}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}\nolimits}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}\nolimits}

\newcommand{\eqdistr}{\stackrel{d}{=}}
\newcommand{\todistr}{\overset{d}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\toweak}{\overset{w}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\toprobab}{\overset{P}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\toas}{\overset{a.s.}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\ton}{\overset{}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\tosquare}{\stackrel{L^2}{\to}}
\newcommand{\bsl}{\backslash}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bu}{\mathbf{u}}


\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bEta}{\boldsymbol{\eta}}
\newcommand{\dd}{{\,\rm d}}

\newcommand{\stirling}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}
\newcommand{\stirlingsec}[2]{\genfrac{\{}{\}}{0pt}{}{#1}{#2}}

\newcommand{\given}{\,|\,}
\newcommand{\bgiven}{\,\big|\,}


